A Nearly Optimal All-Pairs Min-Cuts Algorithm in Simple Graphs

We give an $n^{2+o(1)}$-time algorithm for finding $s$-$t$ min-cuts for all pairs of vertices $s$ and $t$ in a simple, undirected graph on $n$ vertices. We do so by constructing a Gomory-Hu tree (or cut equivalent tree) in the same running time, thereby improving on the recent bound of $\tilde{O}(n^{2.5})$ by Abboud et al. (STOC 2021). Our running time is nearly optimal as a function of $n$.

==> isolate_well_linked.tex <==

\subsection{Proof of \Cref{lem:single-source}}
\label{sec:isolate_well-linked}
A key tool in proving this lemma will be the {\em Isolating Cuts Lemma} from \cite{LiP20deterministic}. 

We restate this lemma below for convenience. \alert{We remark that there is one minor distinction: in our case, we require the $(t,T\setminus\{t\})$-mincuts to be \emph{minimal}.\thatchaphol{Define minimal. Use ``closest-to-$t$'' instead?} However, the exact same proof from \cite{LiP20deterministic} works for this strengthened version of the lemma.}

\begin{lemma}[Isolating Cut Lemma~\cite{LiP20deterministic}]
\label{lem:isolating}
Let $G = (V, E)$ be an undirected graph on $n$ vertices and $m$ edges, and let $T\subseteq V$ be any set of terminal vertices. Then, using $O(\log n)$ maxflow calls each on graphs that have $O(n)$ vertices and $O(m)$ edges in total plus $O(m)$ time, there is an algorithm that finds the \alert{minimal} $(t, T\setminus \{t\})$-mincut for every $t\in T$.\jason{I need the minimal requirement. (Actually, \cite{LiP21approximate} needs it too; it's not there right now, but that needs to be fixed.)}
\end{lemma}

Now, we give a detailed proof of \Cref{lem:single-source}. Note that since $X$ is well-linked in $G$, it follows that a $(p, v)$-mincut for any vertex $v\in X$ is unbalanced in terms of the number of vertices in $X$ that are on either side of the cut. We formalize this below.

\begin{lemma}
\label{lem:unbalanced}
Let $G = (V, E)$ be an undirected graph and $X$ be a $(d, \phi)$-well-linked set of vertices in $V$ such that the value of every $(x, y)$-mincut for $x, y\in X$ is less than $2d$. For any two vertices $p, x\in X$, let $(a, B)$ be a $(p, x)$-mincut. Then, $\min(|A\cap X|, |B\cap X|) \le \frac{2}{\phi}$.
\end{lemma}
\begin{proof}
By the condition of the lemma, the value of a $(p, x)$-mincut is at most $2d$. But, by the well-linkedness of $X$, the value of $(A, B)$ is at least $d\phi\cdot \min(|A\cap X|, |B\cap X|)$. The lemma follows.
\end{proof}


Let us now fix an $(x, y)$-mincut for every $x, y\in X$ and call it $(A_{xy}, B_{xy})$ where $x\in A_{xy}, y\in B_{xy}$. We call the given vertex $p\in X$ the {\em pivot}. %if for at least $\frac{|X|}{4}$ vertices $x\in X$, we have $|A_{xp}\cap X| \le B_{xp}\cap X$. In other words, for at least a quarter of 
The well-linked vertices $X$ can be separated into two categories based on the pivot $p$. If for some vertex $x\in X$, we have $|A_{xp}| \le |B_{xp}|$, i.e., the smaller side in terms of vertices from $X$ in the $(x, p)$-mincut is the one containing $x$, then we say that $x$ is {\em separable} from $p$. On the other hand, if $|A_{xp}| > |B_{xp}|$, i.e., the smaller side in terms of vertices from $X$ in the $(x, p)$-mincut is the one containing $p$, then we say that $x$ is {\em not separable} from $p$. 

\eat{
The next lemma essentially appears in \cite{AbboudKT20}, but we need a slightly more general version and give a proof for completeness.

\begin{lemma}
\label{lem:tournament}
If $p$ is selected uniformly at random from $X$, then it is a pivot with probability at least $1/2$.
\end{lemma}
\begin{proof}
\alert{blah}
\end{proof}
}

%Next, suppose that that we have selected a pivot $p$. Then, 
Our first goal is to identify the $(p, x)$-mincut for vertices $x\in X$ that are separable from $p$. We sample $X$ at rate $\frac{\phi}{2}$ to obtain a set of vertices $S$. The next lemma shows a crucial property of this sample.

\begin{lemma}
\label{lem:sep}
Let $p\in X$ be a pivot, and let $S$ be an i.i.d. sample of $X$ at rate $\frac{\phi}{2}$. Then, for any vertex $x\in X$ that is separable from $p$ where $(A_{xp}, B_{xp})$ is the $(x, p)$-mincut, we have $A_{xp}\cap S = \{x\}$ with probability at least $\frac{\phi}{2e}$.
\end{lemma}
\begin{proof}
For any vertex $x$ that is separable from $p$, we have $|A_{xp}| \le |B_{xp}|$, i.e., the side containing $x$ in the $(x, p)$-mincut is smaller than that containing $p$. By \Cref{lem:unbalanced}, we have $|A_{xp}\cap X| \le \frac{2}{\phi}$. Then, we have $A_{xp}\cap S = \{x\}$ with probability
$$\Pr[x\in S]\cdot \Pr[(A_{xp}\setminus\{x\})\cap S = \emptyset] 
= \frac{\phi}{2}\cdot \left(1-\frac{\phi}{2}\right)^{|A_{xp}|-1} 
\ge \frac{\phi}{2}\cdot \left(1-\frac{\phi}{2}\right)^{\frac{2}{\phi}-1}
\ge \frac{\phi}{2}\cdot \frac{1}{e} 
= \frac{\phi}{2e}.$$ 
\end{proof}

%This lemma is useful for finding the $(p, x)$-mincut for vertices $x$ that are separable from $p$. 
Next, we  consider vertices $x\in X$ that are {\em not} separable from $p$. The next lemma gives a property of the  sample $S$ that is useful for such vertices. 

\begin{lemma}
\label{lem:notsep}
Let $p\in X$ be a pivot, and let $S$ be an i.i.d. sample of $X$ at rate $\frac{\phi}{2}$. Then, for any vertex $x\in X$ that is not separable from $p$ where $(A_{xp}, B_{xp})$ is the $(x, p)$-mincut, we have $x\in S$ and $(B_{xp}\setminus\{p\})\cap S = \emptyset$ with probability at least $\frac{\phi}{2e}$.
\end{lemma}
\begin{proof}
For any vertex $x$ that is not separable from $p$, we have $|A_{xp}| > |B_{xp}|$, i.e., the side containing $p$ in the $(x, p)$-mincut is smaller than that containing $x$. By \Cref{lem:unbalanced}, we have $|B_{xp}\cap X| \le \frac{2}{\phi}$. Then, we have $x\in S$ and $(B_{xp}\setminus \{p\})\cap S = \emptyset$ with probability
$$\Pr[x\in S]\cdot \Pr[(B_{xp}\setminus\{p\})\cap S = \emptyset] 
= \frac{\phi}{2}\cdot \left(1-\frac{\phi}{2}\right)^{|B_{xp}|-1} 
\ge \frac{\phi}{2}\cdot \left(1-\frac{\phi}{2}\right)^{\frac{2}{\phi}-1}
\ge \frac{\phi}{2}\cdot \frac{1}{e} 
= \frac{\phi}{2e}.$$ 
\end{proof}

If the last two lemmas holds, then \Cref{lem:isolating} can be used to identify the $(A_{xp}, B_{xp})$-mincut for vertices $x$ that are separable and not separable from $p$ respectively. We put this together in the next algorithm.

\begin{algorithm}
\begin{enumerate}
\item Initialize a table $\Lambda$ with $|X|-1$ rows to store $(x, p)$-mincuts for every $x\in X$, $x\not= p$
\item Initialize $\Lambda(x) \gets \bot$ for all $x$
\item Repeat $c\cdot \frac{\ln n}{\phi}$ times (for a large enough constant $c$)
\begin{enumerate}
\item Sample $S$ from $X$ i.i.d. at rate $\frac{\phi}{2}$
\item Call the Isolating Cuts Lemma (\Cref{lem:isolating}) on $S\cup \{p\}$ and obtain cuts $C_1, C_2, \ldots$
\item For each $C_i$, 
\begin{enumerate}
    \item If $p\notin C_i$, then for each $x\in X\cap C_i$, update $\Lambda(x)\gets C_i$ if $\delta(C_i) < \delta(\Lambda(x))$
    \item If $p\in C_i$, then for each $x\in X\setminus C_i$, update $\Lambda(x)\gets C_i$ if $\delta(C_i) < \delta(\Lambda(x))$
\end{enumerate}
\end{enumerate}
\item Return $\Lambda$
\end{enumerate}
\caption{\label{alg:ssc}$\protect\ssc(G, p, X)$}
\end{algorithm}

The next lemma uses \Cref{lem:sep} and \Cref{lem:notsep} to establish correctness of \Cref{alg:ssc}.

\begin{lemma}
\label{lem:ssc}
\Cref{alg:ssc} computes whp a $(p, x)$-mincut for every $x\in X$ where $x\not= p$, and uses $O\left(\frac{\polylog(n)}{\phi}\right)$ maxflow calls plus $\Otil\left(\frac{m}{\phi}\right)$ time.
\end{lemma}
\begin{proof}
First, note that irrespective of the samples, the cut $\Lambda(x)$ for any $x$ is a $(x, p)$ cut. Therefore, we only need to show that for each $x$, there is a sample $S$ that reveals the $(x, p)$-mincut. If $x$ is separable, this follows from \Cref{lem:sep}, while if $x$ is not separable, then this follows from \Cref{lem:notsep}. The lemma follows by using a union bound on the vertices $x\in X\setminus \{p\}$.

For the running time bound, note that $O\left(\frac{\log n}{\phi}\right)$ invocations of \Cref{lem:isolating} takes $O\left(\frac{\polylog(n)}{\phi}\right)$ maxflow calls plus $\Otil\left(\frac{m}{\phi}\right)$ time. Additionally, for each invocation of \Cref{lem:isolating}, we update table $\Lambda$ in $O(n)$ time for a total of $\Otil\left(\frac{n}{\phi}\right) = \Otil\left(\frac{m}{\phi}\right)$ time.
\end{proof}

